Multiscale Comparative Connectomics

The connectome, a map of the structural and/or functional connections in the brain, provides a complex representation of the neurobiological phenotypes on which it supervenes. This information-rich data modality has the potential to transform our understanding of the relationship between patterns in brain connectivity and neurological processes, disorders, and diseases. However, existing computational techniques used to analyze connectomes are oftentimes insufficient for interrogating multi-subject connectomics datasets: many current methods are either solely designed to analyze single connectomes or leverage heuristic graph statistics that are unable to capture the complete topology of multiscale connections between brain regions. To enable more rigorous connectomics analysis, we introduce a set of robust and interpretable effect size measures motivated by recent theoretical advances in random graph models. These measures facilitate simultaneous analysis of multiple connectomes across different scales of network topology, enabling the robust and reproducible discovery of hierarchical brain structures that vary in relation to phenotypic profiles. In addition to explaining the theoretical foundations and guarantees of our algorithms, we demonstrate their superiority over current state-of-the-art connectomics methods through extensive simulation studies and real-data experiments. Using a set of high-resolution connectomes obtained from genetically distinct mouse strains (including the BTBR mouse -- a standard model of autism -- and three behavioral wild-types), we illustrate how our methods successfully uncover latent information in multi-subject connectomics data and yield valuable insights into the connective correlates of neurological phenotypes that other methods do not capture. The data and code necessary to reproduce our analyses are available at https://github.com/neurodata/MCC.

==> tables/mdmr_vertex.tex <==
\begin{table*}[ht!]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Vertex}                & \textbf{statistic} & \textbf{p-value} \\ \midrule
Substantia Nigra (L) & 0.855 & 3.28e-05 \\
Middle Cerebellar Peduncle (R) & 0.852 & 3.45e-05 \\
Internal Capsule (L) & 0.851 & 3.5e-05 \\
Substantia Nigra (R) & 0.845 & 3.84e-05 \\
Pontine Reticular Nucleus (R) & 0.840 & 4.14e-05 \\
Pontine Reticular Nucleus (L) & 0.838 & 4.25e-05 \\
Parasubiculum (L) & 0.838 & 4.25e-05 \\
Ventral Tegmental Area (R) & 0.837 & 4.32e-05 \\
Retro Rubral Field (L) & 0.829 & 4.91e-05 \\
Fastigial Medial Nucleus of Cerebellum (R) & 0.824 & 5.3e-05 \\
Cerebral Peduncle (R) & 0.819 & 5.74e-05 \\
Cerebral Peduncle (L) & 0.818 & 5.87e-05 \\
Fastigial Medial Nucleus of Cerebellum (L) & 0.814 & 6.23e-05 \\
Fimbria (L) & 0.813 & 6.28e-05 \\
Brain Stem Rest (L) & 0.811 & 6.46e-05 \\
Cingulate Cortex Area 30 (L) & 0.810 & 6.6e-05 \\
Ventral Tegmental Area (L) & 0.806 & 6.99e-05 \\
Globus Pallidus (R) & 0.802 & 7.46e-05 \\
Internal Capsule (R) & 0.797 & 8.09e-05 \\
Subthalamic Nucleus (R) & 0.792 & 8.78e-05 \\
Zona Incerta (R) & 0.783 & 0.000102 \\
Parabrachial Nucleus (L) & 0.783 & 0.000102 \\
Globus Pallidus (L) & 0.781 & 0.000104 \\
Insular Cortex (R) & 0.780 & 0.000106 \\
Brain Stem Rest (R) & 0.777 & 0.00011 \\
Secondary Visual Cortex Mediolateral Area (R) & 0.777 & 0.00011 \\
Inferior Colliculus (R) & 0.776 & 0.000111 \\
Superior Cerebellar Peduncle (L) & 0.775 & 0.000113 \\
Retro Rubral Field (R) & 0.773 & 0.000117 \\
Stria Terminalis (L) & 0.772 & 0.000118 \\
Postsubiculum (R) & 0.769 & 0.000123 \\
Midbrain Reticular Nucleus (L) & 0.768 & 0.000125 \\
Striatum (R) & 0.768 & 0.000125 \\
Primary Visual Cortex Binocular Area (R) & 0.768 & 0.000125 \\
Corpus Callosum (L) & 0.767 & 0.000125 \\ \bottomrule
\end{tabular}
\caption{The top 34 vertices (out of 326 total vertices) as detected by MDMR, ranked by the order of their Holm--Bonferroni corrected p-values. MDMR is a weak statistical test for detecting signal vertices given that the corpus callosum is the 34th ranked vertex.}
\label{tab:mdmr_vertex}
\end{table*}
